How Far Are We to GPT-4V? Closing the Gap to Commercial Multimodal Models with Open-Source Suites

In this report, we introduce InternVL 1.5, an open-source multimodal large language model (MLLM) to bridge the capability gap between open-source and proprietary commercial models in multimodal understanding. We introduce three simple improvements: (1) Strong Vision Encoder: we explored a continuous learning strategy for the large-scale vision foundation model -- InternViT-6B, boosting its visual understanding capabilities, and making it can be transferred and reused in different LLMs. (2) Dynamic High-Resolution: we divide images into tiles ranging from 1 to 40 of 448$\times$448 pixels according to the aspect ratio and resolution of the input images, which supports up to 4K resolution input. (3) High-Quality Bilingual Dataset: we carefully collected a high-quality bilingual dataset that covers common scenes, document images, and annotated them with English and Chinese question-answer pairs, significantly enhancing performance in OCR- and Chinese-related tasks. We evaluate InternVL 1.5 through a series of benchmarks and comparative studies. Compared to both open-source and proprietary models, InternVL 1.5 shows competitive performance, achieving state-of-the-art results in 8 of 18 benchmarks. Code has been released at https://github.com/OpenGVLab/InternVL.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> table/ablation_component.tex <==
\begin{table}[t]\scriptsize
\renewcommand{\arraystretch}{1.0}
\centering

\setlength\tabcolsep{1.05pt}
\begin{tabular}{lll|c|c|c|ccc}
    visual & glue & \multirow{2}{*}{LLM}  &  \multirow{2}{*}{dataset}   & dialogue & caption & \multicolumn{3}{c}{visual question answering}  \\
    encoder & layer &  &  & MME & NoCaps & OKVQA  & VizWiz$\rm_{val}$ & GQA  \\
    
    \hline

    EVA-E  & MLP & V-7B & 665K~\cite{liu2023improved} & 970.5 & 75.1 & 40.1 & 25.5 & 41.3 \\
    
    IViT-6B & MLP & V-7B & 665K~\cite{liu2023improved} & 1022.3 & 80.8 & 42.9 & 28.3  & 45.8 \\
    
    IViT-6B & QLLaMA & V-7B & 665K~\cite{liu2023improved} & 1227.5 & 94.5 & 51.0 & 38.4 & 57.4 \\

    \hline
    
    IViT-6B & QLLaMA & V-7B & Ours & 1298.5 & 120.5 & 51.8 & 44.9 & 57.7 \\

    IViT-6B & QLLaMA & V-13B & Ours & 1317.2 & 123.1 & 55.5 & 55.7 & 59.5 \\
    
    
\end{tabular}
\vspace{-0.5em}
\caption{
\textbf{Ablation of InternVL's feature representations.}
V-7B and V-13B denote Vicuna-7B and Vicuna-13B \cite{zheng2023vicuna}, respectively.
}
\vspace{-0.5em}
\label{tab:ablation_component}
\end{table}

==> table/data_intro_stage1_2.tex <==
\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.1}
    \centering

    \setlength\tabcolsep{5pt}
    \begin{tabular}{p{3.2cm}|p{13.5cm}}
        dataset & introduction  \\
        \hline

    \multicolumn{2}{l}{\emph{Training Data for Stage 1 \& Stage 2.}}    \\ 
    
    LAION-en~\cite{schuhmann2022laion5b} &  LAION-en is a part of the LAION-5B dataset, containing 2.32 billion English-only image-text pairs.  \\
    
    \rowcolor{gray!15}
    LAION-multi~\cite{schuhmann2022laion5b} & LAION-multi is another segment of LAION-5B, featuring 2.26 billion image-text pairs across more than 100 languages, and is ideal for multilingual studies. \\
    
    Laion-COCO~\cite{schuhmann2022laioncoco} & Laion-COCO comprises 663 million synthetic captions for web images, generated using a blend of BLIP-L/14 \cite{li2022blip} and CLIP models \cite{radford2021clip}.  \\
    
    \rowcolor{gray!15}
    COYO~\cite{byeon2022coyo} &  COYO-700M is a large-scale dataset that contains 747 million image-text pairs as well as many other meta-attributes to increase the usability to train various models. It follows a similar strategy to previous vision-language datasets, collecting many informative pairs of alt-text and its associated image in HTML documents.  \\
    
    Wukong~\cite{gu2022wukong} & Wukong is a large-scale Chinese image-text dataset for benchmarking different multi-modal pre-training methods. It contains 100 million Chinese image-text pairs from the web. \\

    \rowcolor{gray!15}
    CC3M~\cite{sharma2018cc3m} & This dataset consists of approximately 3 million images, each annotated with a caption.  \\
    
    CC12M~\cite{changpinyo2021cc12m} &  CC12M is a dataset with 12 million image-text pairs. It is larger and covers a much more diverse set of visual concepts than the CC3M \cite{sharma2018cc3m}.  \\

    \rowcolor{gray!15}
    SBU~\cite{ordonez2011sbu} &  The SBU Captioned Photo Dataset is a collection of over 1 million images with associated text descriptions extracted from Flicker. \\

    \hline
    \multicolumn{2}{l}{\emph{Testing Datasets for Image Classification.}}    \\ 

    ImageNet-1K \cite{deng2009imagenet} & A large-scale dataset commonly used in image classification, consisting of over 1 million images across 1K different classes. \\

    \rowcolor{gray!15}
    ImageNet-ReaL \cite{beyer2020imagenetreal} & It contains ImageNet val images augmented with a new set of ``re-assessed" labels. These labels are collected using an enhanced protocol, resulting in multi-label and more accurate annotations. \\
    
    ImageNet-V2 \cite{recht2019imagenetv2} & A dataset created to test the robustness of models trained on ImageNet-1K, containing new test images collected following the original methodology. \\

    \rowcolor{gray!15}
    ImageNet-A \cite{hendrycks2021imagenet_a} & It consists of real-world, unmodified, and naturally occurring examples that are misclassified by ResNet models \cite{he2016deep}. It's designed to highlight the challenges of adversarial examples in natural settings. \\
    
    ImageNet-R \cite{hendrycks2021imagenet_r} & A set of images labeled with ImageNet labels obtained by collecting art, cartoons, deviantart, graffiti, embroidery, graphics, origami, paintings, patterns, plastic objects, plush objects, sculptures, sketches, tattoos, toys, and video game renditions of ImageNet classes. It has renditions of 200 ImageNet classes resulting in 30K images.  \\

    \rowcolor{gray!15}
    ImageNet-Sketch \cite{wang2019imagenet_sketch} & It consists of 51K images, approximately 50 images for each of the ImageNet classes. It is constructed using Google Image queries with the standard class name followed by ``sketch of". \\
    
    ObjectNet \cite{barbu2019objectnet} &
    ObjectNet is a crowd-sourced test set of 50K images featuring objects in unusual poses and cluttered scenes, designed to challenge recognition performance. It includes controls for rotation, background, and viewpoint, and covers 313 object classes, with 113 overlapping with ImageNet \cite{deng2009imagenet}. \\

    \rowcolor{gray!15}
    Multilingual IN-1K \cite{laion_ai_2023_clip} & An adaptation of ImageNet-1K supporting multilingual annotations, facilitating research in cross-lingual image classification. \\
    
    CIFAR-10/100 \cite{krizhevsky2009cifar} & It comprises 60K 32$\times$32 images in 10 classes (CIFAR-10) or 100 classes (CIFAR-100). \\

    \rowcolor{gray!15}
    MNIST \cite{lecun1998mnist} & A classic dataset containing 70K 28$\times$28 gray-scale images of handwritten digits. \\

    Caltech-101 \cite{fei2004learning} &
    The dataset comprises images of objects from 101 classes and a background clutter class, each labeled with a single object. It contains about 40 to 800 images per class, totaling approximately 9K images. \\

    \rowcolor{gray!15}
    SUN397 \cite{xiao2010sun} & The SUN397 or Scene UNderstanding (SUN) is a dataset for scene recognition consisting of 397 categories with 109K images. \\

    FGVC Aircraft \cite{maji2013fgvc} & The dataset contains 10K images of aircraft, with 100 images for each of 102 different aircraft model variants, most of which are airplanes. \\

    \rowcolor{gray!15}
    Country-211 \cite{radford2021clip} & It is a dataset released by OpenAI, designed to assess the geolocation capability of visual representations. It filters the YFCC100M \cite{thomee2016yfcc100m} dataset to find 211 countries that have at least 300 photos with GPS coordinates. OpenAI built a balanced dataset with 211 categories, by sampling 200 photos for training and 100 photos for testing, for each country. \\

    Stanford Cars \cite{krause2013cars} & This dataset consists of 196 classes of cars with a total of 16K images, taken from the rear. The data is divided into almost a 50-50 train/test split with 8K training images and 8K testing images. \\ 

 
    \end{tabular}
    \caption{\textbf{Introduction of datasets used in InternVL's stage 1 and stage 2.}
    In summary, we utilize a vast amount of image-text data for pre-training and conduct comprehensive evaluation across a wide range of generic visual-linguistic tasks.
}
\label{tab:data_intro_stage1_2_page1}
\end{table*}

\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.1}
    \centering

    \setlength\tabcolsep{5pt}
    \begin{tabular}{p{3.2cm}|p{13.5cm}}
        dataset & introduction  \\
        \hline

    \multicolumn{2}{l}{\emph{Testing Datasets for Image Classification.}}    \\ 
    
    Birdsnap \cite{berg2014birdsnap} & Birdsnap is a large bird dataset consisting of 49,829 images from 500 bird species with 47,386 images used for training and 2,443 images used for testing.
    Due to broken links, we are only able to download 1,845 out of the 2,443 testing images.  \\

    \rowcolor{gray!15}
    DTD \cite{cimpoi2014d2d} & The Describable Textures Dataset (DTD) contains 5,640 texture images in the wild. They are annotated with human-centric attributes inspired by the perceptual properties of textures. \\
    
    Eurosat \cite{helber2019eurosat} & This dataset is based on Sentinel-2 satellite images covering 13 spectral bands and consisting of 10 classes with 27K labeled and geo-referenced samples. \\

    \rowcolor{gray!15}
    FER2013 \cite{goodfellow2013fer2013} &
    This dataset includes around 30K RGB facial images, categorized into seven expressions: angry, disgust, fear, happy, sad, surprise, and neutral.  \\
    
    Flowers-102 \cite{nilsback2008flowers} & It is consistent with 102 flower categories commonly occurring in the United Kingdom. Each class consists of between 40 and 258 images.\\

    \rowcolor{gray!15}
    Food-101 \cite{bossard2014food101} & The Food-101 dataset consists of 101 food categories with 750 training and 250 test images per category, making a total of 101K images.\\
    
    GTSRB \cite{stallkamp2012gtsrb} & The German Traffic Sign Recognition Benchmark (GTSRB) contains 43 classes of traffic signs, split into 39,209 training images and 12,630 test images.  \\

    \rowcolor{gray!15}
    Pets \cite{parkhi2012cats} & The Oxford-IIIT Pet Dataset is a 37-category pet dataset with roughly 200 images for each class created by the Visual Geometry Group at Oxford. \\
    
    Rendered SST2 \cite{radford2021clip} & This dataset is used to evaluate the model's capability on optical character recognition. It was generated by rendering sentences in the Standford Sentiment Treebank v2 dataset. \\
    
    \rowcolor{gray!15}
    Resisc45 \cite{coates2011stl10} & This is a dataset for remote sensing scene classification. It contains 31,500 RGB images divided into 45 scene classes, each class containing 700 images. \\
    
    STL10 \cite{nilsback2008flowers} & The STL-10 dataset, inspired by CIFAR-10~\cite{krizhevsky2009cifar}, includes 10 classes with 500 training and 800 test color images each, sized 96$\times$96 pixels.   \\

    \rowcolor{gray!15}
    VOC2007 \cite{everingham2015pascal} &
    The Pascal VOC 2007 dataset focuses on recognizing objects in realistic scenarios and contains 20 object classes across 9,963 images with 24,640 labeled objects. The data has been divided into 50\% for training/validation and 50\% for testing. Following common practice, we conduct zero-shot image classification by cropping images to isolate objects using bounding boxes.\\
    
    \hline
    \multicolumn{2}{l}{\emph{Testing Datasets for Video Classification.}}    \\ 
    
    Kinetics 400 \cite{carreira2017k400} & A large-scale dataset containing around 400 human action classes with at least 400 video clips for each class, sourced from YouTube. \\

    \rowcolor{gray!15}
    Kinetics 600 \cite{carreira2018k600} & An expansion of Kinetics 400, this dataset includes 600 action classes and provides an increased diversity in video representation.  \\

    Kinetics 700 \cite{carreira2019k700} & The latest in the series, Kinetics 700 offers an even broader range with 700 action categories, further challenging the robustness of retrieval models.  \\
    
    \hline
    \multicolumn{2}{l}{\emph{Testing Datasets for Image-Text Retrieval.}}    \\ 

    COCO \cite{chen2015cococaption} & The COCO Caption dataset contains diverse images with detailed captions, widely used for image-text retrieval and image captioning tasks. \\

    \rowcolor{gray!15}
    COCO-CN \cite{li2019cococn} & COCO-CN is a bilingual image description dataset enriching COCO with manually written Chinese sentences and tags. The new dataset can be used for multiple tasks including image tagging, captioning, and retrieval, all in a cross-lingual setting. \\
    
    Flickr30K \cite{plummer2015flickr30k} & This dataset comprises 31,000 images sourced from Flickr, each annotated with five captions, making it suitable for image-text retrieval. \\

    \rowcolor{gray!15}
    Flickr30K-CN \cite{lan2017flickrcn} & Flickr30K-CN offers Chinese captions for the images, enabling studies in cross-lingual and multi-modal retrieval tasks. \\
    
    XTD \cite{aggarwal2020xtd} & A newly developed 1K multilingual test set, featuring COCO images annotated in various languages.  \\

    \hline
    \multicolumn{2}{l}{\emph{Testing Dataset for Video-Text Retrieval.}}    \\ 

    MSR-VTT \cite{xu2016msrvtt} &  This is a large-scale dataset for open-domain video captioning and video-text retrieval, comprising 10,000 video clips across 20 categories. Each clip is annotated with 20 English sentences, totaling about 29,000 distinct words in all captions. The standard division of the dataset allocates 6,513 clips for training, 497 for validation, and 2,990 for testing purposes. \\
    
    \end{tabular}
    \caption{\textbf{Introduction of datasets used in InternVL's stage 1 and stage 2.} 
    In summary, we utilize a vast amount of image-text data for pre-training and conduct comprehensive evaluation across a wide range of generic visual-linguistic tasks.
}
\label{tab:data_intro_stage1_2_page2}
\end{table*}


\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.1}
    \centering

    \setlength\tabcolsep{5pt}
    \begin{tabular}{p{3.2cm}|p{13.5cm}}
        dataset & introduction  \\
        \hline

    \multicolumn{2}{l}{\emph{Testing Datasets for Image Captioning.}}    \\ 
    
    COCO \cite{chen2015cococaption} & We use the Karpathy test set for testing. \\

    \rowcolor{gray!15}
    Flickr30K \cite{plummer2015flickr30k} & We use the Karpathy test set for testing. \\ 
    
    NoCaps  \cite{agrawal2019nocaps} & NoCaps stands out for testing models' capabilities in open-ended caption generation, using images that go beyond the training data's domain. We report the performance on the NoCaps val set. \\
    
    \hline
    \multicolumn{2}{l}{\emph{Testing Dataset for Semantic Segmentation.}}    \\ 

    ADE20K \cite{zhou2017ade20k} & ADE20K contains more than 20K scene-centric images exhaustively annotated with pixel-level objects and object parts labels. There are a total of 150 semantic categories, which include stuffs like sky, road, grass, and discrete objects like person, car, bed. We report the performance on the ADE20K val set. \\
    
    \end{tabular}
    \caption{\textbf{Introduction of datasets used in InternVL's stage 1 and stage 2.} 
    In summary, we utilize a vast amount of image-text data for pre-training and conduct comprehensive evaluation across a wide range of generic visual-linguistic tasks.
}
\label{tab:data_intro_stage1_2_page3}
\end{table*}

\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.15}
    \centering

    \setlength\tabcolsep{5pt}
    \begin{tabular}{p{3.2cm}|p{13.5cm}}
        dataset & introduction  \\
        \hline

    \multicolumn{2}{l}{\emph{Training Data for SFT.}}    \\ 
    
    COCO Caption \cite{chen2015cococaption} & It contains over 0.5 million captions describing over 110K images. Following common practice, we use the Karpathy training set for training. We transform it into a dialogue dataset using the response formatting prompt: ``Provide a one-sentence caption for the provided image." \\

    \rowcolor{gray!15}
    TextCaps \cite{sidorov2020textcaps} & TextCaps contains 145K captions for 28K images. It challenges a model to recognize text, relate it to its visual context, and decide what part of the text to copy or paraphrase. OCR tokens are used during training.  We transform it into a dialogue dataset using the response formatting prompt: ``Provide a one-sentence caption for the provided image." \\
    
    VQAv2 \cite{goyal2017vqav2} & VQAv2, the second version of the VQA dataset, features open-ended questions related to images. Answering these questions demands a grasp of vision, language, and common sense.  We convert it into a dialogue dataset using the prompt: ``Answer the question using a single word or phrase."\\

    \rowcolor{gray!15}
    OKVQA \cite{marino2019okvqa} & A dataset with over 14K questions requiring external knowledge for answers, focusing on knowledge-based visual question answering. We transform it into a dialogue dataset using the response formatting prompt: ``Answer the question using a single word or phrase." \\

    A-OKVQA \cite{schwenk2022aokvqa} & An augmented successor of OKVQA \cite{marino2019okvqa} and contains 25K questions requiring a broad base of commonsense and world knowledge to answer.  We transform it into a dialogue dataset using the response formatting prompt: ``Answer with the option’s letter from the given choices directly." \\

    \rowcolor{gray!15}
    IconQA \cite{lu2021iconqa} & A dataset with 107K questions across three sub-tasks, focusing on abstract diagram recognition and comprehensive visual reasoning. We convert it into a dialogue dataset using these prompts: ``Answer with the option’s letter from the given choices directly." and ``Answer the question using a single word or phrase." \\
    
    AI2D \cite{kembhavi2016ai2d} & AI2D features over 5K grade school science diagrams with rich annotations and 15K multiple-choice questions for diagram understanding research. We convert it into a dialogue dataset using the prompt: ``Please answer the question based on the options mentioned before."\\

    \rowcolor{gray!15}
    GQA \cite{hudson2019gqa} & GQA is a large-scale dataset with more than 110K images and 22 million questions, combining real images with balanced question-answer pairs for visual reasoning.  We transform it into a dialogue dataset using the prompt: ``Answer the question using a single word or phrase." \\
    

    OCR-VQA~\cite{mishra2019ocrvqa} & The OCR-VQA dataset contains 207,572 images of book covers and more than 1 million question-answer pairs about these images. We convert it into a dialogue dataset using the response formatting prompt: ``Answer the question using a single word or phrase." \\

    \rowcolor{gray!15}
    ChartQA~\cite{masry2022chartqa} & ChartQA is a dataset for question answering about charts, focusing on visual and logical reasoning. It comprises 9.6K human-written questions and 23.1K questions generated from human-written chart summaries.  We convert it using the prompt: ``Answer the question using a single word or phrase."  \\
    
    DocVQA~\cite{clark2017docqa} & The DocVQA dataset consists of 50,000 questions defined on over 12,000 document images. We convert it into a dialogue dataset using the prompt: ``Answer the question using a single word or phrase." \\

    \rowcolor{gray!15}
    ST-VQA~\cite{biten2019stvqa} & The ST-VQA dataset contains a total of 31,791 questions over 23,038 images. The training set alone consists of 26,308 questions based on 19,027 images. We convert it into a dialogue dataset using the response formatting prompt: ``Answer the question using a single word or phrase." \\

    \end{tabular}
    \caption{\textbf{Introduction of datasets used in InternVL's stage 3.} 
    We collect a wide range of high-quality instruction data. For non-dialogue datasets, we follow the response formatting prompts described in \cite{liu2023improved} for conversion. Note that only the training set is used for training.
}
\label{tab:data_intro_stage3_page1}
\end{table*}

\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.1}
    \centering

    \setlength\tabcolsep{5pt}
    \begin{tabular}{p{3cm}|p{13.7cm}}
        dataset & introduction  \\
        \hline

    \multicolumn{2}{l}{\emph{Training Data for SFT.}}    \\ 


    EST-VQA~\cite{wang2020estvqa} & The EST-VQA dataset provides questions, images, and answers, but also a bounding box for each question that indicates the area of the image that informs the answer.  We convert it into a dialogue dataset using the response formatting prompt: ``Answer the question using a single word or phrase." \\

    \rowcolor{gray!15}
    InfoVQA~\cite{mathew2022infographicvqa} & This dataset includes a diverse collection of infographics with natural language questions and answers. It focuses on reasoning over document layout, textual content, graphical elements, and data visualizations. We convert it into a dialogue dataset using the prompt: ``Answer the question using a single word or phrase."  \\

    LLaVAR~\cite{zhang2023llavar} & The LLaVAR dataset advances visual instruction tuning for Large Language Models by focusing on text-rich images. It incorporates 422K images processed with OCR and 16K GPT-4 generated conversations, enhancing text-based VQA performance and human interaction capabilities in diverse scenarios. Note that, we only use the 20K high-quality data for fine-tuning of LLaVAR. \\

    \rowcolor{gray!15}
    RefCOCO \cite{yu2016refcoco, mao2016refcocog} & A mixed dataset of RefCOCO~\cite{yu2016refcoco}, RefCOCO+\cite{yu2016refcoco}, and RefCOCO-g~\cite{mao2016refcocog}. We convert it into a dialogue dataset following LLaVA-1.5 \cite{liu2023improved}. \\

    Toloka \cite{ustalov2023toloka} & The TolokaVQA dataset comprises images with associated textual questions, each marked with a bounding box indicating the visual answer. It's sourced from a licensed subset of the COCO dataset and labeled on the Toloka platform. We convert it into a dialogue dataset following LLaVA-1.5 \cite{liu2023improved}. \\

    \rowcolor{gray!15}
    LLaVA-150K~\cite{liu2023llava} & This is a set of GPT-generated multi-modal instruction-following data, constructed for visual instruction tuning and building large multi-modal models towards GPT-4 vision/language capability. It includes 158K unique language-image instruction-following samples.  \\

    SVIT \cite{zhao2023svit} & This dataset includes 3.2 million visual instruction tuning data, with 1.6M conversation QA pairs, 1.6M complex reasoning QA pairs, and 106K detailed image descriptions. It is designed to improve multi-modal performance in visual perception, reasoning, and planning. For this dataset, we merge the QA pairs from the same training image into a single conversation. \\

    \rowcolor{gray!15}
    VisDial \cite{das2017visdial} & A dataset based on the COCO images, featuring dialogues created by two Amazon Mechanical Turk workers. One plays the `questioner', seeing only an image's text description, and the other, the `answerer', sees the image. They engage in a 10-round Q\&A session about the image. \\

    LRV-Instruction \cite{liu2023lrv-instruction} & 
    The LRV-Instruction dataset is designed to combat hallucination in large multi-modal models. It comprises 120K GPT-4-generated visual instructions for 16 vision-and-language tasks, including both positive and negative instructions for robust tuning. Negative instructions focus on Nonexistent and Existent Element Manipulation. This dataset helps improve accuracy and consistency in multi-modal tasks. \\

    \rowcolor{gray!15}
    LLaVA-Mix-665K \cite{liu2023improved} & LLaVA-Mix-665K is an instruction-following dataset mixed from 10 academically oriented datasets. \\

    \hline
    \multicolumn{2}{l}{\emph{Testing Dataset for SFT (Image Captioning).}}    \\ 
    COCO \cite{chen2015cococaption} & Karpathy test set is used for testing. The prompt is: ``Provide a one-sentence caption for the provided image.'' \\

    \rowcolor{gray!15}
    Flickr30K \cite{plummer2015flickr30k} & Karpathy test set is used for testing. The prompt is: ``Provide a one-sentence caption for the provided image.''  \\ 
    
    NoCaps  \cite{agrawal2019nocaps} & NoCaps val set is used for testing. The prompt is: ``Provide a one-sentence caption for the provided image.''  \\
    

    \hline
    \multicolumn{2}{l}{\emph{Testing Dataset for SFT (Visual Question Answering).}}    \\ 
    VQAv2~\cite{goyal2017vqav2} & VQAv2 test-dev set is used for testing. The prompt is: ``Answer the question using a single word or phrase.'' \\

    \rowcolor{gray!15}
    GQA~\cite{hudson2019gqa} & GQA test-balanced set is used. The prompt is: ``Answer the question using a single word or phrase.'' \\
    
    VizWiz~\cite{gurari2018vizwiz} & VizWiz test-dev set is used for testing. The prompt is: ``When the provided information is insufficient, respond with `Unanswerable'. Answer the question using a single word or phrase.'' \\

    \rowcolor{gray!15}
    TextVQA~\cite{singh2019textvqa} & TextVQA val set is used for testing. The prompt is: ``Answer the question using a single word or phrase.'' \\

    \hline
    \multicolumn{2}{l}{\emph{Testing Dataset for SFT (Multi-Modal Dialogue).}}    \\ 
    MME~\cite{fu2023mme} & MME is a comprehensive evaluation benchmark for multi-modal large language models. It measures both perception and cognition abilities on a total of 14 subtasks, including existence, count, position, color, poster, celebrity, scene, landmark, artwork, OCR, commonsense reasoning, numerical calculation, text translation, and code reasoning. The prompt for this dataset is: ``Answer the question using a single word or phrase.'' \\

    \rowcolor{gray!15}
    POPE~\cite{li2023pope} & POPE is a popular dataset used to evaluate object hallucination. The response formatting prompt used for this dataset is: ``Answer the question using a single word or phrase.'' \\

    
    \end{tabular}
    \caption{\textbf{Introduction of datasets used in InternVL's stage 3.}
    We collect a wide range of high-quality instruction data. For non-dialogue datasets, we follow the response formatting prompts described in \cite{liu2023improved} for conversion. Note that only the training set is used for training.
    We evaluate our InternVL-Chat models on three tasks, including image captioning, VQA, and multi-modal dialogue.
    For these datasets, we employ the same response formatting prompts as for LLaVA-1.5~\cite{liu2023improved}.
}
\label{tab:data_intro_stage3_page2}
\end{table*}

==> table/dataset.tex <==
\begin{table}[ht]\scriptsize
    \centering
    \begin{subtable}{0.53\linewidth}  % 创建第一个子表格，占据页面宽度的一半
        \centering
        \setlength\tabcolsep{1pt}
        \renewcommand{\arraystretch}{1.05}
      \begin{tabular}{l|cccccc|c|c}
        method &  IN-1K &  IN-A &  IN-R &  IN-V2 &  IN-Ske &  ObjectNet & $\Delta${$\downarrow$} & avg. \\
        \hline

         OpenCLIP-H &
         78.0 &  59.3 &  89.3 &  70.9 &  66.6 &  69.7 & 5.7 &  72.3\\
         
         OpenCLIP-g & 
         78.5 &  60.8 &  90.2 &  71.7 &  67.5 &  69.2 & 5.5 &  73.0 \\
         
         OpenAI CLIP-L+ &
         76.6 &  77.5 &  89.0 &  70.9 &  61.0 &  72.0 & 2.1 &  74.5 \\
         
         EVA-01-CLIP-g &
         78.5 &  73.6 &  92.5 &  71.5 &  67.3 &  72.3 & 2.5 &  76.0 \\
         
         OpenCLIP-G & 
         80.1 &  69.3 &  92.1 &  73.6 &  68.9 &  73.0 & 3.9 &  76.2\\
         
         EVA-01-CLIP-g+ & 
         79.3 &  74.1 &  92.5 &  72.1 &  68.1 &  75.3 & 2.4 &  76.9\\
         
         EVA-02-CLIP-L+ &
         80.4 &  82.9 &  93.2 &  73.8 &  68.9 &  78.4 &  \textbf{0.8} &  79.6 \\
         
         EVA-02-CLIP-E &
         81.9 &  80.4 &  94.1 &  75.4 &  71.8 &  76.9 &  1.8 &  80.1\\
         
         EVA-02-CLIP-E+ & 
         82.0 &  82.1 &  94.5 &  75.7 &  71.6 &  79.6 &  1.1 &  80.9\\

         \textcolor{gray}{CoCa$^\dagger$} & 
         \textcolor{gray}{86.3} &  \textcolor{gray}{90.2} &  \textcolor{gray}{96.5} &  \textcolor{gray}{80.7} &  \textcolor{gray}{77.6} &  \textcolor{gray}{82.7} & \textcolor{gray}{0.6}  &  \textcolor{gray}{85.7} \\

        \hline
         \rowcolor{gray!20}
         InternVL-CLIP &
         \textbf{83.2} &	\textbf{83.8} &	\textbf{95.5} &	\textbf{77.3} &	\textbf{73.9} &	\textbf{80.6} &	\textbf{0.8} &  \textbf{82.4} \\
    \end{tabular}
        \caption{ImageNet variants and ObjectNet.}
        \label{subtable:a}
    \end{subtable}%
    \vspace{0.5em}
    \begin{subtable}{0.46\linewidth}  % 创建第一个子表格，占据页面宽度的一半
        \centering
        \setlength\tabcolsep{3pt}
        \renewcommand{\arraystretch}{1.05}
      \begin{tabular}{l|ccccc|c}
        method &  EN &  ZH &  JP &  AR &  IT &  avg. \\

        \hline
        CLIP-Italian  &
        $-$	& $-$ & $-$ & $-$ & 22.1 & $-$ \\

        Japanese-CLIP-ViT-B &
        $-$	& $-$ & 54.6 & $-$ & $-$ & $-$ \\
        
        Taiyi-CLIP-ViT-H &
        $-$	& 54.4 & $-$ & $-$ & $-$ & $-$ \\

        WuKong-ViT-L-G &
        $-$	& 57.5 & $-$ & $-$ & $-$ & $-$ \\

        WuKong-Swin-L &
        $-$	& 58.2 & $-$ & $-$ & $-$ & $-$ \\
        
        CN-CLIP-ViT-H &
        $-$	& 59.6 & $-$ & $-$ & $-$ & $-$ \\

        AltCLIP-ViT-L &
        74.5 & 59.6 & $-$ & $-$ & $-$ & $-$ \\

        EVA-02-CLIP-E+ & 
        82.0 & 3.6 & 5.0 & 0.2 & 41.2 & 26.4 \\

        
        OpenCLIP-XLM-R-B &
        62.3 &	42.7 &	37.9 &	26.5 &	43.7 &	42.6  \\

        OpenCLIP-XLM-R-H &
        77.0 &	55.7 &	53.1 &	37.0 &	56.8 &	55.9  \\
        
        \hline
         \rowcolor{gray!20}
         InternVL-CLIP &
         \textbf{83.2} &	\textbf{64.5} &	\textbf{61.5} &	\textbf{44.9} &	\textbf{65.7} &	\textbf{64.0}  \\
    \end{tabular}
        \caption{Multilingual ImageNet-1K.}
        \label{subtable:a}
    \end{subtable}%
    \vspace{-0.5em}
    \caption{\textbf{Comparison of zero-shot image classification performance.} 
    ``{$\Delta$\scriptsize$\downarrow$}'': The gap between the averaged top-1 accuracy and the IN-1K top-1 accuracy. 
    $^\dagger$ CoCa~\citep{yu2022coca} uses the JFT-3B dataset~\citep{zhai2022scaling} with label names for pretraining.
    Multilingual evaluation involves 5 languages, including English (EN), Chinese (ZH), Japanese (JP), Arabic (AR), and Italian (IT).
    }
    \vspace{-0.5em}
    \label{table:main}
\end{table}

==> table/model_config.tex <==
\begin{table}[tp]
\scriptsize
\renewcommand\arraystretch{1.0} % Line spacing
    \centering
    \setlength\tabcolsep{6.1pt}
    \vspace{0.5em}
    \begin{tabular}{l|cccc|c}
        name & width & depth & MLP & \#heads & \#param (M) \\
        \hline

        ViT-G~\cite{zhai2022scaling} & 1664 & 48 & 8192 & 16 & 1843 \\
        
        ViT-e~\cite{chen2022pali} & 1792 & 56 & 15360 & 16 & 3926 \\

        EVA-02-ViT-E~\cite{sun2023evaclip} & 1792 & 64 & 15360 & 16 & 4400 \\

        ViT-6.5B~\cite{singh2023maws} & 4096 & 32 & 16384 & 32 & 6440 \\
        ViT-22B~\cite{dehghani2023vit22b} & 6144 & 48 & 24576 & 48 & 21743 \\

        \rowcolor{gray!15}
        InternViT-6B (ours) & 3200 & 48 & 12800 & 25 & 5903 \\

    \end{tabular}
\vspace{-0.5em}
\caption{\textbf{Architecture details of the InternViT-6B model.}
\vspace{-0.5em}
}
\label{tab:model_config}
\end{table}

==> table/retrieval_ft_config.tex <==
\begin{table}[t]
\scriptsize
\renewcommand{\arraystretch}{1.0}
    \centering
    \setlength\tabcolsep{4pt}
    \begin{tabular}{l|c}
        config & retrieval fine-tuning  \\
        \hline
        image-text data & ~~~~~~~Flickr30K \cite{plummer2015flickr30k} / Flickr30K-CN \cite{lan2017flickrcn}~~~~~~~ \\
        peak learning rate & 1e-6 \\
        layer-wise lr decay rate & InternViT-6B (0.9), QLLaMA (0.9) \\
        learning rate schedule & cosine decay \\
        optimizer & AdamW~\cite{loshchilov2017adamw}  \\
        optimizer hyper-parameters & $\beta_{1}$, $\beta_{2}$ = 0.9, 0.999\\
         weight decay & 0.05 \\
         input resolution & 364$^2$ \\
         patch size & 14  \\
         total batch size & 1024 \\
         warm-up iterations & 100 \\
         training epochs & 10 \\
         drop path rate~\cite{huang2016droppath} & 0.3  \\
         data augmentation & random resized crop \& flip \\
         numerical precision & DeepSpeed bf16~\cite{rasley2020deepspeed}\\
          trainable / total parameters~~~~~~ & 14B / 14B \\
          GPUs for training & 32$\times$A100 (80G) \\
          
    \end{tabular}
    \caption{\textbf{Training settings of retrieval fine-tuning.} 
    We fine-tune InternVL on Flickr30K and Flickr30K-CN separately.
}
\label{tab:train_cfg_ft_retrieval}
\end{table}

==> table/small_medium_large_table.tex <==
\begin{figure*}[t]\centering
\begin{minipage}{0.46\linewidth}\vspace{0mm}    
    \centering
    \scriptsize
    \begin{tcolorbox}[boxrule=0.2mm]
        \centering
        \hspace{-5mm}
        \begin{tabular}{p{0.99\columnwidth}}
        \hspace{1mm}
        \begin{minipage}{0.99\columnwidth}
        
        \includegraphics[width=.85\linewidth]{figure/Localization_1.jpg}  

        \textbf{User:} Tell me the locations of all the number 10 jerseys in the picture.
        \vspace{4px}

        \textbf{GPT-4V:} In the image, there are two players wearing number 10 jerseys. The first one is located towards the center, slightly to the right while facing the image; he's wearing a red jersey and is the second person from the right in the group wearing red and white uniforms. The second player is wearing a light blue jersey and is positioned on the far left side of the image; he's the third person from the left in the group wearing blue and white uniforms. 
        \vspace{4px}
        
        \textbf{InternVL 1.5:} In the image, there are two number 10 jerseys visible:
        1.The first player wearing the number 10 jersey is located in the center of the image. He is wearing a red jersey with the number 10 on it, and he is standing with his hands on his hips.
        2.The second player with the number 10 jersey is on the far right of the image. He is wearing a blue jersey with the number 10 on it and is crouching down with his hands on his knees. 
        
        \end{minipage}
        \end{tabular}
    \end{tcolorbox}
\end{minipage}
\hspace{2em}
\begin{minipage}{0.46\linewidth}\vspace{0mm}    
    \centering
    \scriptsize
    \begin{tcolorbox}[boxrule=0.2mm]
        \centering
        \hspace{-5mm}
        \begin{tabular}{p{0.99\columnwidth}}
        \hspace{1mm}
        \begin{minipage}{0.99\columnwidth}
        
        \includegraphics[width=.8\linewidth]{figure/Localization_2.png} 

        \textbf{User:} What is the man in the picture doing with his right hand?
        \vspace{4px}

        \textbf{GPT-4V:} The man in the picture is pointing with his right hand towards a beluga whale that appears to be behind a glass barrier. He seems to be doing this to show the whale to the child he is holding, likely to engage the child's interest or to teach the child about the whale.
        \vspace{4px}
        
        \textbf{InternVL 1.5:} The man in the picture is pointing at a large dolphin through a glass barrier. He is likely making this gesture to draw attention to the dolphin, either for the child he is holding or for others around them. This could be to educate the child about the dolphin, to highlight a specific behavior or feature of the dolphin, or simply to share the experience with others. The gesture is a common way to direct someone's attention to something of interest. 
        
        \end{minipage}
        \end{tabular}
    \end{tcolorbox}
\end{minipage}
\caption{\textbf{Examples for Object Localization.} 
\textcolor{blue}{Blue} highlights the standout answers.
}
\label{fig:localization}
\end{figure*}

==> table/stage12_data.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \renewcommand\arraystretch{1.0} % Line spacing
    \setlength{\tabcolsep}{1.1mm}    % table col width
    \begin{tabular}{l|cc|cc|cc}
          & \multicolumn{2}{c|}{characteristics} & \multicolumn{2}{c|}{stage 1}  & \multicolumn{2}{c}{stage 2} \\
         \multirow{-2}{*}{dataset} & language & original & cleaned & remain  & cleaned & remain \\
         \hline
         LAION-en~\cite{schuhmann2022laion5b}  & \multirow{6}{*}{English} & 2.3B & 1.94B & 84.3\% &  91M & 4.0\% \\
         LAION-COCO~\cite{schuhmann2022laioncoco}  &  & 663M     & 550M   & 83.0\% & 550M & 83.0\% \\
         COYO~\cite{byeon2022coyo}        &  & 747M     & 535M   & 71.6\% & 200M & 26.8\% \\
         CC12M~\cite{changpinyo2021cc12m}       &  & 12.4M      & 11.1M  & 89.5\% & 11.1M  & 89.5\% \\
         CC3M~\cite{sharma2018cc3m}        &  & 3.0M       & 2.6M   & 86.7\% & 2.6M   & 86.7\%  \\
         SBU~\cite{ordonez2011sbu}
         &  & 1.0M & 1.0M & 100\% & 1.0M & 100\% \\
         
         \rowcolor{gray!15}
         Wukong~\cite{gu2022wukong}& \multirow{1}{*}{Chinese} & 100M  & 69.4M & 69.4\% & 69.4M & 69.4\% \\
         
         LAION-multi~\cite{schuhmann2022laion5b} & \multirow{1}{*}{Multi} & 2.2B  & 1.87B & 85.0\% & 100M & 4.5\%\\
         \hline
          Total      &  Multi & 6.03B     & 4.98B    & 82.6\% & 1.03B & 17.0\%\\
    \end{tabular}
    \vspace{-0.5em}
    \caption{\textbf{Details of the training data for \modelname in stage 1 and stage 2.}
    Among them, LAION-en~\cite{schuhmann2022laion5b}, LAION-multi~\cite{schuhmann2022laion5b}, COYO~\cite{byeon2022coyo}, and Wukong~\cite{gu2022wukong} are web-scale image-text pairs data.
    LAION-COCO~\cite{schuhmann2022laioncoco} is a synthetic dataset with high-quality captions from LAION-en. CC12M~\cite{changpinyo2021cc12m}, CC3M~\cite{sharma2018cc3m}, SBU~\cite{ordonez2011sbu} are academic caption datasets. ``Multi" means multilingual.
    } 
    \vspace{-0.5em}
    \label{tab:stage1_data}
\end{table}

==> table/train_config.tex <==
\begin{table}[t]
\scriptsize
\renewcommand{\arraystretch}{1.0}
    \centering

    \setlength\tabcolsep{4pt}
    \begin{tabular}{l|cc}
        config & stage 1 & stage 2 \\
        \hline

        image enc. weight init. & random init.~\cite{bao2021beit} & from stage 1  \\
        text enc. weight init. & from~\cite{cui2023chinesellama} & from stage 1  \\
        image enc. peak learning rate & 1e-3 & frozen \\
        text enc. peak learning rate & 1e-4 & frozen \\
        cross attn peak learning rate & -- & 5e-5 \\
        learning rate schedule & cosine decay & cosine decay \\
        optimizer & AdamW~\cite{loshchilov2017adamw} & AdamW~\cite{loshchilov2017adamw} \\
        optimizer hyper-parameters & $\beta_{1}$, $\beta_{2}$ = 0.9, 0.95 & $\beta_{1}$, $\beta_{2}$ = 0.9, 0.98 \\
         weight decay & 0.1 & 0.05 \\
         input resolution & 196$^2$ $\rightarrow$ 224$^2$ & 224$^2$ \\
         patch size & 14 & 14 \\
         total batch size & 164K & 20K \\
         warm-up iterations & 5K & 2K \\
         total iterations & 175K & 80K \\
         samples seen & 28.7B & 1.6B \\
         drop path rate~\cite{huang2016droppath} & uniform (0.2) & 0.0 \\
         data augmentation & random resized crop & random resized crop \\
         numerical precision & DeepSpeed bf16~\cite{rasley2020deepspeed} & DeepSpeed bf16~\cite{rasley2020deepspeed} \\
          trainable / total parameters & 13B / 13B & 1B / 14B \\
          GPUs for training & 640$\times$A100 (80G) & 160$\times$A100 (80G) \\
    \end{tabular}
    \caption{\textbf{Training settings of InternVL's stage 1 and stage 2.} 
    ``196$^2$ $\rightarrow$ 224$^2$" means we initially train at a 196$\times$196 resolution, and later switch to 224$\times$224 resolution for the final 0.5 billion samples, for higher training efficiency.
}
\label{tab:train_cfg_stage1_stage2}
\end{table}

==> table/zero-shot-vqa.tex <==
\begin{table*}[t]\scriptsize
\renewcommand{\arraystretch}{1.0}
\begin{subtable}{1\textwidth}
    \centering
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
        & \multicolumn{3}{c|}{Image Captioning} & \multicolumn{7}{c}{Visual Question Answering} \\
        & COCO & Flickr30k & NoCap & VQAv2 & OKVQA & VizWiz &  GQA  & VisDial  & TextVQA & SciQA  \\
        method & karpathy test & karpathy test     &  val  & test-dev &  test  & test-dev & test-dev & val & test &  \\
        \hline
        
        
        Flamingo-9B~\cite{alayrac2022flamingo} & 
        79.4 & 61.5 & $-$ & 51.8 & 44.7 & 28.8 & $-$ & 48.0 & 31.8 & $-$ \\
        
        Flamingo-80B~\cite{alayrac2022flamingo} & 
        84.3 & 67.2 & $-$ & 56.3/82.0$^*$ & 50.6 & 31.6 & $-$ & 52.0 & 35.0 & $-$ \\
        
        SimVLM~\cite{wang2021simvlm} & 
        143.3$^*$  & $-$  & 112.2 & 80.0$^*$  & $-$  & $-$  & $-$  & $-$ & $-$ & $-$ \\
        
        CoCa~\cite{yu2022coca} &
        143.6$^*$  & $-$  & 122.4 & 82.3$^*$  & $-$  & $-$  & $-$  & $-$ & $-$ & $-$ \\
        
        BLIP~\cite{li2022blip} & 
        136.7$^*$  & $-$  & 113.2 & 78.3$^*$  & $-$  & $-$  & $-$  & 69.4$^*$  & $-$ & $-$ \\
        
        BLIP-2~\cite{li2023blip2} & 
        144.5$^*$  & $-$  & 121.6 & 65.0/82.2$^*$ & 45.9 & $-$  & 44.7 & $-$ & 42.4 & $-$ \\

        InstructBLIP (Vicuna-7B)~\cite{instructblip} & 
        $-$  & 82.4 & 123.1 & $-$  & $-$  & 34.5 & 49.5  & 48.5 & 50.7 & \\
        
        InstructBLIP (Vicuna-13B)~\cite{instructblip} & 
        $-$  & 82.8 & 121.9 & $-$  & $-$  & 34.5 & 49.5  & 48.5 & 50.7 & \\
        
        Shikra-13B (Vicuna-13B)~\cite{chen2023shikra} &
        117.5$^*$  & 73.9 &  $-$  & 77.4$^*$  & 47.2 & $-$  & $-$  & $-$ & $-$ & $-$\\
        
        KOSMOS-1~\cite{huang2023kosmos1} & 
        84.7 & 67.1 &  $-$  & 51.0 & $-$  & 29.2 & $-$  & $-$ \\
        
        KOSMOS-2~\cite{peng2023kosmos2} & 
        $-$  & 66.7 &  $-$  & 45.6 & $-$  & $-$  & $-$  & $-$ \\
        
        
        Emu~\cite{sun2023emu} & 
        112.4 & $-$ &  $-$  & 52.0 & 38.2 & 34.2 & $-$  & 47.4 & $-$ \\
        
        Emu-I~\cite{sun2023emu} & 
        117.7 & $-$ &  $-$  & 40.0 & 34.7 & 35.4 & $-$  & 48.0 & $-$ \\
        
        DreamLLM~\cite{dong2023dreamllm} & 
        115.4 & $-$ &  $-$  & 56.6 & 44.3 & 38.1 & $-$  & $-$ & 34.9 \\
        
        Qwen-VL~\cite{bai2023qwen} & 
        $-$ & 85.8 & 121.4 & 79.5$^*$ & 58.6$^*$ & 35.2 & 59.3$^*$ & $-$ & 63.8 & 67.1 \\
        
        Qwen-VL-Chat~\cite{bai2023qwen} &
        $-$ & 81.0 & 120.2 & 78.2$^*$ & 56.6$^*$ & 38.9 & 57.5$^*$ & $-$ & 61.5 & 68.2 \\
        
        LLaVA-1.5 \\
        
        \rowcolor{gray!15}
        InternVL-QLLaMA &
        \textbf{128.2} & 79.2 & 113.7 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\  

        \rowcolor{gray!15}
        InternVL-Chat &
        &  &  &  &  &  &  &  &  &  \\  
        
         
    \end{tabular}
\end{subtable}
\caption{\textbf{Comparison of image captioning and visual question answering.}
$^\dagger$These models are finetuned with the COCO dataset and zero-shot transferred to other datasets.
}
\label{tab: zs_cap_vqa}
\end{table*}
